DEL: Discrete Element Learner for Learning 3D Particle Dynamics with Neural Rendering

Learning-based simulators show great potential for simulating particle dynamics when 3D groundtruth is available, but per-particle correspondences are not always accessible. The development of neural rendering presents a new solution to this field to learn 3D dynamics from 2D images by inverse rendering. However, existing approaches still suffer from ill-posed natures resulting from the 2D to 3D uncertainty, for example, specific 2D images can correspond with various 3D particle distributions. To mitigate such uncertainty, we consider a conventional, mechanically interpretable framework as the physical priors and extend it to a learning-based version. In brief, we incorporate the learnable graph kernels into the classic Discrete Element Analysis (DEA) framework to implement a novel mechanics-integrated learning system. In this case, the graph network kernels are only used for approximating some specific mechanical operators in the DEA framework rather than the whole dynamics mapping. By integrating the strong physics priors, our methods can effectively learn the dynamics of various materials from the partial 2D observations in a unified manner. Experiments show that our approach outperforms other learned simulators by a large margin in this context and is robust to different renderers, fewer training samples, and fewer camera views.

==> sec/X_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We briefly and accurately conclude the contribution and scope of our proposed paper in the abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discussed the limitations of our proposed method in Section.\ref{Conclusion&Limitation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper provides the full set of assumptions and a complete proof and introduction in Section.\ref{sec: Method}, and \ref{sec. experiment}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In this paper, we give a detailed introduction about how we construct the dataset. The proposed method, training, and testing paradigm, and data collection method are completely reproducible and easy to follow.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code and dataset can be obtained by emailing the author only for research collaborations. One can also easily reproduce the proposed physics-informed GNN on the guidance of the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We give implementation details, comparative experiments, and ablation studies in Section.\ref{sec. experiment}, and our Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We give qualitative and quantitative experimental results to prove our proposed method outperforms existing dynamic learners across multiple scenarios in Section~\ref{sec. experiment} and the Appendix. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The information on computing resources is concluded in the \textbf{Appendix}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our proposed methods, code, datasets, and experiment paradigms fully comply with NeurIPS' Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the potential impact of this work in the Appendix. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for the responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In this paper, we do not utilize datasets with a high risk of misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The creators and original owners of assets used in the paper are all credited and the license and terms of use are explicitly mentioned and properly respected.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not contain crowdsourcing experiments and research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sec/X_suppl_grain.tex <==
\clearpage
% \setcounter{page}{1}
\onecolumn
\appendix
\part*{Appendix}
\section{Nomenclature}
We list all symbols and marks used in the main paper in the following Table for the convenience of reference. %\ref{table: nomenclature}

\begin{longtable*}
\renewcommand{\arraystretch}{0.96}
\setlength\tabcolsep{10.5mm}{
\begin{tabular}{cl}
\hline\hline
\textbf{Variable}   & \textbf{Description} \\
\hline
$i$      & i-th particle\\
$\mathbf{x}_i$      & position vector of particle\\
$\mathbf{v}_i$      & velocity vector of particle\\
$\mathbf{a}_i$      & acceleration vector of particle\\
$\mathbf{u}_i$      & movement vector of particle\\
$F^p_{ij}$          & potential interaction force\\
$F^v_{ij}$          & viscous force\\
$F^g_i$             & gravity\\
$\mathbf{F}^{pn}_{ij}$    & potential interaction force vector along the normal direction\\
$\mathbf{F}^{pt}_{ij}$    & potential interaction force vector along the tangential direction\\
$\mathbf{F}^{vn}_{ij}$    & viscous interaction force vector along the normal direction\\
$\mathbf{F}^{vt}_{ij} $   & viscous interaction force vector along the tangential direction\\
$\delta d_n$    & intrusion scalar\\
$\delta d_t$    & instantaneous tangential displacement\\
$\Delta t$    & time interval \\
$r_i$      & radius of particle\\
$A_i$    & attribute of i-th particle\\
$F^b_{ij}$    & bond particle between particles which belong to the same object      \\
$\mathcal{F}^n_c$& mapping from intrusion scalar and attributes of particles to normal contact force\\
$\mathcal{F}^t_c$ & mapping from intrusion scalar and attributes of particles to tangential contact force\\
$\mathcal{F}^n_v$ & mapping from intrusion scalar and attributes of particles to normal viscous force\\
$\mathcal{F}^t_v$ & mapping from intrusion scalar and attributes of particles to tangential viscous force\\
$\mathcal{F}^n_b$ & mapping from intrusion scalar and attributes of particles to normal bond force\\
$\mathcal{O}_k $    & set of particles belonging to the same k-th object\\
$\mathbf{v}^t_{ij} $    & the tangential velocity vector\\
$\mathbf{n}$      & normal unit vector\\
$\mathbf{t} $     & tangential unit vector\\
$\phi^n$      & the normal dissipative model\\
$\phi^t$      & the tangential dissipative model\\
$\Phi^n$     & normal graph kernel\\
$\Phi^t$     & tangential graph kernel\\
$\mathcal{H}_c$      & prediction head to regress the magnitude of the contact forces\\
$\mathcal{H}_b$      & prediction head to regress the magnitude of the bond forces\\
$\sigma$  & sigmoid activation function\\
$f^{bn}_{ij}$      & the normal bond force\\
$f^{bt}_{ij}$      & the tangential bond force\\
$f^{cn}_{ij}$      & the normal contact force\\
$f^{ct}_{ij}$      & the tangential contact force\\
$f^{n'}_{ij} $    & precomputed normal force vector\\
$\mathbf{f}^n_{ij} $    & normal force vector\\
$f^{t'}_{ij}$    & precomputed tangential force\\
$\mathbf{f}^t_{ij}  $   & tangential force vector\\
$\mu  $   & the frictional coefficient\\
$n_i $     & i-th node features\\ 
$v_i(t)$  & velocity of i-th particle at timestep $t$\\ 
$h_i$     & latent embedding from i-th particle attribute\phantom{ of particles to tangential contact force}\\
$e_{ij} $  & edge features between node $i$ and $j$\\
\hline\hline
\end{tabular}}
\label{tab: nomenclature}
\end{longtable*}

\begin{multicols}{2}
% \twocolumn
\section{Detailed architecture}
% \cref{fig: point renderer} gives detailed information about the point-based renderer. This figure describes the post-process after aggregating features from neighboring points. It is observed that the aggregated features are fed to their corresponding decoders. The color decoder integrates the positional embedding of the view direction with the shape decoder's hidden vector. Both decoders are structured as MLPs with dual hidden layers, each comprising 128 neurons. After deriving $\sigma$ and $c$, conventional volume rendering techniques are employed to compute pixel colors.

% The MNGO's architectural nuances are detailed next. Its graph operator is illustrated from Eq. 8 to Eq. 12 in our main manuscript. The operator components, denoted as $\phi$s, are realized using MLPs. The $\varphi_{vn}$ and $\varphi_{vt}$ components, representing viscous elements, are dependent solely on their respective velocity magnitudes. These are modeled using a simple MLP architecture with two layers of 200 neurons each, incorporating a sigmoid activation function prior to coefficient output and reflecting the viscous forces' role in diminishing contact forces. In contrast, the $\varphi_{pn}$ and $\varphi_{pt}$ components have distinct objectives, aiming to map the constitutive relationship from relative mapping to pair-wise forces. This involves accounting for relative invasions and individual particle attributes, as detailed in Eq. 5 to Eq. 8 of our main paper. The embedding vectors for per-particle attributes, denoted as $m_i$ and $m_j$, are defined as $\mathbf{h}=[mat, ||a_i^{t-1}||_2]$, where $mat$ signifies the material type and $||a_i^{t-1}||_2]$ represents the particle's acceleration magnitude at the preceding timestamp.
We describe the detailed architecture used in the MNGO. The entire graph operator is depicted in Equation~\ref{eq: embedding} to Equation~\ref{eq: tangential disspative mechanism} in the main paper. 

The embedding layer is an MLP with 2 hidden layers. The output embedding latent vector is normalized to [-1,1]. The $A_i$ and $A_j$ refer to the embedding vectors of the per-particle attribute, which we define as $A=[mat, ||a_i^{t-1}||_2]$. Here the $mat$ denotes the type of materials, $||a_i^{t-1}||_2]$ represents the value of the acceleration at the last timestamp of this particle. We use a simple MLP with two hidden layers (each layer includes 200 neurons) to model $\phi^t$ and $\phi^n$. Also, the sigmoid activation is used before outputting the coefficients because the viscous forces are manifested as a reduction in potential interaction forces.

The $\Phi^{n}$ and $\Phi^{t}$ aim to map related physical quantities to the abstracted node and edge features which we implement by a 3-layer MLP of 200 hidden dimensions with residual connection and Layer Normalization. The abstracted features then are input to two different output heads $\mathcal{H}_b, \mathcal{H}_c$ to produce the final magnitude of the forces. We call the $\Phi^*$ MNGO Abstraction layer and the $\mathcal{H}_*$ MNGO Output layer. Notably, only the particle $i$, $j$ belong to the same object, the $\mathcal{H}_b$ will be activated, otherwise the $f_{ij}^b$ will be set to zero constantly. 
% For the $\Phi^{n}$ and $\Phi^{t}$, also and their associated prediction heads, $\mathcal{H}_b, \mathcal{H}_c$, the two functions aim to model the physical quantities to the pair-wise forces. We call the two $\Phi^*$ as MNGO Abstraction layer and all $\mathcal{H}_*$ as MNGO Output layer. The details are as follows. 

% The GNN kernel's representational capabilities are augmented through multistep message passing. Notably, the final step in our GNN kernel holds physical meanings and cannot be input for subsequent GNN layers. Therefore, we introduce two different types of GNN layers, including the MNGO Abstraction layer and the MNGO Output layer. The abstraction layer aims to abstract hidden vectors from the raw node input to a latent space. Once abstraction within this latent domain is complete, the output layer then translates these hidden variables into the magnitude of interaction forces. We describe the process in the following Algorithm. 
% \begin{algorithm}
% \KwData{attributes $A$, accelerations $\mathbf{a}$, edge unit vector $\mathbf{e}_{ij}$, edge vector properties $\mathbf{E}_{ij}$}
% \KwResult{interaction forces}
% $h_i \leftarrow \text{embedding}(\text{A}_i)$\;
% $h_j \leftarrow \text{embedding}(\text{A}_j)$\;
% $\mathbf{H}_{i} \leftarrow \mathbf{a}_i$, $\mathbf{H}_{j} \leftarrow \mathbf{H}_j$\;
% \For{$l$ in [Abstraction layers]}
% {$H_{ij},\,h_{ij} \leftarrow G_{a,m-p}(m_i,\,||\mathbf{M}_i||_2,\,m_j,\,||\mathbf{M}_j||_2, ||\mathbf{E}_{ij}||_2)$\;
% $\mathbf{E}_{ij} \leftarrow M_{ij}\mathbf{e}_{ij}$\;
% $\mathbf{M}^{'}_{i} \leftarrow \sum\limits_{j \in \mathcal{N}}M_{ij}\mathbf{e}_{ij} $\;
% $m^{'}_{i} \leftarrow \sum\limits_{j \in \mathcal{N}}m_{ij}+m_i $\;
% $C_{i},\,m_{i} \leftarrow G_{a,a}(||\mathbf{M}^{'}_{i}||_2,\,||\mathbf{M}_i||_2,\,m^{'}_{i},\,m_{i})$\;
% $\mathbf{M}_i = C_i[\mathbf{M}_i, \mathbf{M}^{'}_{i}]^\top$
% }
% $\mathbf{a}_i \leftarrow \mathbf{M}_{i}$;
% $\mathbf{a}_j \leftarrow \mathbf{M}_{j}$\;
% Input to the MNGO Output layer (Eq. 8 - 12 in the main paper);
% \caption{Pseudocode to describe the data stream in MNGO}
% \label{pseudocode}
% \end{algorithm}

% In the \cref{pseudocode}, $A_*$ refers to the attribute of each particle, namely the material type. $attr$ is first embedded by an MLP to a hidden vector with 64 dimensions. The node feature referred by $m_i$ in the main paper is actually the combination of the $m_i$ and $||M_i||$ in Algorithm 1, i.e. a hidden vector with 65 dimensions. For simplicity, we only note the feature as $m_i$ in Equations of the main paper.  
% The $G_{a,m-p}$ denotes the message-passing function of the abstraction layer, and the $G_{a,a}$ denotes the aggregation function. $||E_{ij}||_2$ represents the corresponding edge vectors. For Eq. 8, it refers to the $\delta\mathbf{d}_n$. For Eq. 10, it refers to the $\mathbf{v_{ijt}}$ and $\mathbf{f_{ijn}}$.  It can be seen in the abstraction layer, after aggregating all messages by sum operation, we use another MLP to produce the updated node information. Bold notations represent vectors throughout the algorithm. The two networks only produce scalar to maintain their SE(3) equivariance. $G_{a,m-p}$ deliver the magnitude of the vector messages $M_{ij}$ that multiply with the predefined unit vectors ($\mathbf{n}$ and $\mathbf{t}$ in Eq. 6 and 7 in the main paper). In addition, the output $C_i$ of the $G_{a,a}$ function is a set of coefficients to linearly combine the $\mathbf{M}_i$ and $\mathbf{M}_i^{'}$ to yield the updated node information $||\mathbf{M}_i||_2$ for the next step of message passing. 

% After the last abstraction layer is performed, its output will be fed to the Output layer that decodes the hidden vector to the physical interactions. Each MLP in the process contains two hidden layers with 200 neurons as well. 



\section{Implementation Details}
In this section, we introduce the implementation details of our experiment setup. We first use a pretrained GPF to initialize the scene as particles. 

For the dynamic module, we build the graph at each timestamp via the k-nearest neighbor search with a fixed radius of 0.025. The particle radius ($r$ for different materials) is set to equal the search radius initially and will be optimized through the training process to be a property of the material. In addition, we place a heavy rigid table at the bottom of each scenario, which is also represented by particles but we do not update its position, and its velocity is constantly set to zero. The only function of it is to support the moving objects above. Additionally, the mass parameter for each particle is set to initialize at 1 and optimized during the training phase as well. All models are trained via AdamW optimizer with 5e-4 learning rate. We adopt the StepLR schedule to adjust the learning rate with the increasing step. After 10,000 iterations, we multiply the learning rate by 0.9. After the Equation~\ref{eq: embedding} to Equation~\ref{eq: tangential disspative mechanism} are conducted, we obtain the resultant force of each particle which is divided by its corresponding mass to obtain the acceleration at the current timestamp. Thus we can update their positions by the Euler integration:
\begin{equation}
    \mathbf{v}_{t} = \mathbf{v}_{t-1}+\frac{\mathbf{f}_i}{m_i}\Delta t
\end{equation}
\vspace{-2mm}
\begin{equation}
    \mathbf{x}_t=\mathbf{x}_{t-1}+(\mathbf{v}_{t-1}+\frac{\mathbf{f}_i}{m_i}\Delta t)\Delta t.
\end{equation}
% As for the experimental setting, we compare our method with four baselines. For the dynamic prediction, we simply changed our MNGO module with the EGNN and SGNN simulators that we describe in the main paper because the two simulators are designed for the particle-based dynamic learner when the 3D groundtruth is given. W additionally e reconstruct the dynamic scene by DeVRF method which is a popular NeRF tool specifically for dynamic reconstruction. It utilizes the "static->dynamic" paradigm. In other words, it needs a static initialization first of all, then build a ray bending volume to warp the static initialization into subsequent time. Therefore, we specifically provide 64 camera views at the initial timestamp for DeVRF. Besides, we compare ours with the Neurofluid method, we also use the NeRF-style technique to bridge 2D and 3D and learn particle dynamics directly from images. However, it is limited to simulating liquid material, therefore we only test the comparison on our Fluids scenario. We load the pretrained weights introduced in the Neurofluid and finetune the model on the new scene. 
\section{Detailed Dataset Description}
% In this section, we in detail introduce the data generation of our experiments. We use the Material Point Method to simulate various materials and their interactions. To include different material pairs, we build six different scenarios, namely Plasticine, Multi-Objs, Bear, FluidR, SandFall, and Fluids. Each scenario contains 128 different dynamic episodes for training with different initial conditions. For example, they have various initial shapes, and velocities. However, the material properties, such as their elastic modules or viscosity coefficients, remain the same for the same scenarios. Next, we use SplashSurf to reconstruct meshes and use Blender to render them to obtain the multiview dynamical image sequences. At each timestamp, there are 4 cameras to record the motion. Our target is to learn the material interaction behaviors from those 2D observations. 
In this section, we thoroughly describe the data generation process for our experiments, employing the Material Point Method (MPM) to simulate interactions among various materials. We designed six distinct scenarios to encompass a diverse range of material combinations: Plasticine, Multi-Objs, Bear, FluidR, SandFall, and Fluids. Each scenario is represented through 128 dynamic episodes, differentiated by unique initial conditions such as shapes and velocities, while maintaining consistent material properties, including elasticity and viscosity coefficients, within each scenario.

For the reconstruction of meshes from simulation data, we utilized SplashSurf, followed by rendering multiview dynamic image sequences using Blender. At every timestep, the motion is captured from four distinct camera angles. The objective of this research is to derive material interaction behaviors from these 2D observational sequences.

\noindent \textbf{Plasticine.} This scenario features interactions between two distinct materials: a red elastic object and a blue elastoplastic material. We initialize the elastoplastic materials in various shapes, including duck and bunny configurations, which are then subjected to impacts from the red elastic ball from multiple directions.

\noindent \textbf{Multi-Objs.} This scenario encompasses interactions among five objects composed of three distinct materials. The blue ball and cuboid are categorized as rigid. In contrast, the cylinder and rainbow-colored ring are elastic, each characterized by unique values of elastic modulus and Poisson's ratio. The experimental setup initiates with the rigid ball colliding with the rigid cuboid, triggering a sequence of subsequent collisions. Each episode is distinguished by varying arrangements and initial configurations of the objects, showcasing diversity in shape and positioning.
\end{multicols}
\twocolumn
\noindent \textbf{Bear.} This scenario investigates interactions among objects composed of three distinct materials: plastic, elastic, and rigid. The setup includes a brown bear modeled as a plastic toy, a triangular ship constructed from an elastic material, and a heavy, rigid, yellow box. The experimental design involves the ship and box colliding with the plastic bear from various directions and positions, aiming to study the resultant material behavior and object interactions under different impact scenarios. Each collision is designed to explore the dynamic responses of plastic, elastic, and rigid materials when subjected to varying forces and angles of impact.

\noindent \textbf{Fluids.} The Fluids scenario examines the dynamics of fluid behavior as it impacts a tabletop, with the fluid initially shaped into complex geometries, including forms reminiscent of a bunny, Pokémon, or duck, each varying in size. This setup facilitates observations of the fluid's response upon collision with the ground, encapsulated within a scenario that includes invisible boundaries to constrain the fluid's spread. Upon contacting these boundaries, fluid particles alter their trajectories, enabling detailed study of fluid dynamics and boundary interactions. This scenario allows for the exploration of fluid behavior under varied initial conditions, contributing to our understanding of fluid dynamics in controlled environments.

\noindent \textbf{FluidR.} In this scenario, we explore the dynamics of liquid flow over a hollow shelf with a complex geometry. Across different episodes, we systematically vary the initial configurations of the liquid, altering both its shape and the height from which it is released atop the shelf. The shelf itself is constructed from a hard elastic material, characterized by a very high Young's modulus, to study the interaction between the liquid's fluid dynamics and the shelf's structural response. This setup provides a unique opportunity to observe the behavior of liquids in contact with elastic materials under varying initial conditions, offering insights into fluid-structure interaction phenomena.

\noindent \textbf{SandFall.} This scenario investigates the dynamic interaction between a life buoy, composed of sand soil, and an elastic toy duck. Upon impact, the toy duck undergoes deformation and subsequently recovers to its original shape, causing the sand soil life buoy to rebound. A significant challenge in modeling the dynamics of this interaction lies in the partial obscuration of the toy duck by the sand soil during impact. This obscuration results in incomplete information regarding the duck's deformation and response, complicating the task of accurately learning the system's dynamics. The study focuses on understanding and overcoming the limitations imposed by insufficient visual information on the elastic response of the toy under the impact of granular material. 



% \section{Formulation of Motion Equations}
% As noted in Section 3 of the main paper, in the framework of explicit formulation, the pair-wise particle interaction is defined by a Newton-Euler motion equation:

% \begin{equation}
% M_i\frac{d^2\mathbf{u}}{dt^2}=\mathbf{F}_i=\sum_{j\in \mathcal{N}}(\mathbf{F}^p_{ij}+\mathbf{F}^v_{ij})
%     \label{eq: motion eq1}
% \end{equation}
% % \vspace{-5mm}
% \begin{equation}
% \mathbf{F}^p_{ij}=\mathbf{F}^{pn}_{ij}+\mathbf{F}^{pt}_{ij}
%     \label{eq: motion eq2}
% \end{equation}
% % \vspace{-5mm}
% \begin{equation}
% \mathbf{F}^v_{ij}=\mathbf{F}^{vn}_{ij}+\mathbf{F}^{vt}_{ij}
%     \label{eq: motion eq3}
% \end{equation}
% % \vspace{-5mm}
% \begin{equation}
% M_i\frac{d^2\mathbf{u}}{dt^2}=\sum^N_{j=1}(\mathbf{F}^{n}_{ij}+\mathbf{F}^{t}_{ij})
%     \label{eq: motion eq4}
% \end{equation}
% \begin{equation}
%    M_i\frac{d^2\mathbf{u}}{dt^2} =\sum^N_{j=1}(\mathbf{F}^{pn}_{ij}+\mathbf{F}^{vn}_{ij}) + \sum^N_{j=1}(\mathbf{F}^{pt}_{ij}+\mathbf{F}^{vt}_{ij})
%     \label{eq: motion eq5}
% \end{equation}
% in which $F_i$ can be recognized as the resultant force applied to particle $i$ and the other notations follow the same meaning introduced in the main paper. Here we simply omit the rotation of particles due to its less influence and the gravitational item for simplicity. First, the resultant forces can be considered as the summation of (1) the pair-wise interactions that are caused by deformations and (2) the viscosity resulting from the relative velocities. Conventionally dissipative contributions to interaction force in the pair of discrete elements take into account kinetic energy dissipation mechanisms concerned with the dispersion of elastic waves (this kind of dissipation is general for all solids and liquids). Both terms can be represented as the summation of interactions of all neighbor particles. For each pair, we decompose the two main constituents into the normal and tangential directions, as stated \cref{eq: motion eq2} and \cref{eq: motion eq3}.

% Then we recombine these items according to their directions to derive \cref{eq: motion eq4} and \cref{eq: motion eq5}. Associated with our main paper, we use Eq. 8 and Eq. 9 to model the first term in \cref{eq: motion eq5} and use Eq. 10 and 11 to model the second term. 

% \section{Further Explanation about the Method}
% It is observed from Eq. 6 in the main paper that the pair-wise interaction forces include two components, the contact forces and the bond forces. The contact force exists in any contacted pair of particles while the bond force only exists in the pair of particles where the cohesion exists, which depends on the certain types of materials. Both of the two forces are affected by the relative positions and material properties of the two particles. Due to the similarities of these two forces, such as their formation and direction, we simply use one MLP to model the two interaction behaviors simultaneously, i.e. Eq. 8 in the main paper. 

% Likewise, as for the tangential interaction forces, the components not only contain the above two forces but also a friction term, as stated in Eq. 7 in the main paper. The friction term is affected by the $\mu$ that is associated with the nature of the material and the normal stress. We simply consider all the factors in a unified MLP in Eq. 10 and 11 in the main paper.
%------------------------------------------------------------------------
\section{Additional Results and Comparisons}
% \twocolumn
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{icml2024/Figure/view.pdf}
    \vspace{-5mm}
    \caption{Detailed example of exchanging materials without retraining the model on the SandFall scenario}
    \vspace{-5mm}
    \label{fig: number of input views}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{icml2024/Figure/renderPSNR.pdf}
    \vspace{-5mm}
    \caption{Experiments of the rendering quality of different renderers on Multi-objs dataset. The y coordinate refers to the PSNR metrics.}
    \vspace{-5mm}
    \label{fig: different renderer psnr}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{icml2024/Figure/renderLOGCD.pdf}
    \vspace{-3mm}
    \caption{Experiments of the dynamic prediction of different renderers on Multi-objs dataset. The y coordinate refers to the log Chamber Distance metrics.}
    \vspace{-1mm}
    \label{fig: different renderer log cd}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{icml2024/Figure/datasize.pdf}
    \vspace{-3mm}
    \caption{Experiments of the effect of the number of training episodes on Multi-objs dataset. The x coordinate is the number of training data, and the y coordinate is the log Chamber Distance.}
    \vspace{-3mm}
    \label{fig: training set size}
\end{figure}
\subsection{The influence of different renderer}
The default renderer utilized in the main paper is the GPF. In this section, we evaluate our methods and the baselines with the other two particle-based renderers, i.e. PhysNeRF \cite{guan2022neurofluid}, ParticleNeRF \cite{abou2022particlenerf}, both of which can render dynamic particles. PhysNeRF is employed in Neurofluid to represent and render scenes. However, in the original paper, it is jointly trained with the dynamics module and requires more camera views. For a fair comparison, we pretrain the PhysNeRF from scratch and freeze its parameters for all models. In addition, we provide an initialized particle set for PhysNeRF and ParticleNeRF because they are difficult to initialize the scenes as point clouds from sparse camera views (4 in our experiments), while GPF is capable of initialization due to its depth estimation module. Fig.~\ref{fig: different renderer psnr} and Fig.~\ref{fig: different renderer log cd} show the rendering and dynamic prediction results of different renders. We can see our method achieves better performance regardless of which renderer is employed. Moreover, rendering capability scales proportionally with the accuracy of learned dynamics. As GPF produces better rendering quality, more accurate dynamics can be learned by utilizing it. This example illustrates that our method is robust to the renderer selection because physical priors always guide the model toward a reasonable learning target.  
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figure/sup1.pdf}
    \caption{Long-term predictions of the dynamic NeRF method, the baseline GNN simulators, and our MNGO method on different scenarios.}
    \label{fig: vissup 1}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figure/sup2.pdf}
    \caption{Long-term predictions of the dynamic NeRF method, the baseline GNN simulator, and our MNGO method on different scenarios.}
    \label{fig: vissup 2}
\end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{icml2024/Figure/liquidsup.pdf}
    \vspace{-3.3mm}
    \caption{Qualitative Comparisons of all baselines on Fluids dataset in both rendering and particle views. }
    \vspace{-2.3mm}
    \label{fig: liquidsup}
\end{figure*}
\begin{figure*}[htb]
    \centering
    \includegraphics[width=\linewidth]{Figure/changemat1.pdf}
    \vspace{-3.3mm}
    \caption{Detailed example of swapping materials without retraining the model on the FluidR scenario}
    \vspace{-5mm}
    \label{fig: change 1}
\end{figure*}
\begin{figure*}[htb]
    \centering
    \includegraphics[width=\linewidth]{Figure/changemat2.pdf}
     \vspace{-2.3mm}
    \caption{Detailed example of swapping materials without retraining the model on the SandFall scenario}
    \vspace{-2.3mm}
    \label{fig: change 2}
\end{figure*}
\subsection{The influence of the number of camera views in training}
In this section, we use various numbers of camera views to train the models. In the main paper, four camera views are deployed across four corners of the scene. Here we additionally evaluate if 1, 2, 6, 8, 10 cameras are used, what will happen? The ablation results on Multi-Objs dataset are reported in Fig~\ref{fig: number of input views}. It is observed that our approach is not sensitive to the number of cameras, even if only one camera is used, due to the physical constraints posed by our mechanics framework. The search space is contracted by the physical knowledge injected into the model. Therefore our method can be effectively trained via only visible particles while the invisible ones are constrained through physics. On the contrary, the other two baselines are severely affected by the number of cameras. They cannot learn well from sparse cameras. With the increase in the number of cameras, their performance also improved and the upward trend shows no signs of abating. We can assume that the maximum upper bound of such improvement should be the performance when the 3D labels are used to train them. 

\subsection{The influence of different sizes of training samples}
We evaluate how the training set size affects the performance and the results are reported in Fig,~\ref{fig: training set size}. With increasing sizes of the training set, the log Chamber Distance of EGNN$^*$ and SGNN$^*$ experience slight rises. But our performance remains stable and always stays on top, which means our method is not sensitive to the training sizes and can learn from sparse data. 

\subsection{How does the performance when 3D groundtruth particle labels is used}
We here report the evaluation of training these models with 3D particle tracks. Even though our approach aims to learn 3D dynamics from images, the mechanics-encoded paradigm is also helpful for learning from 3D labels. Table~\ref{tab: 3D gt is given}. show the rollout mean square errors of the three models in all scenarios. From this comparison, SGNN's performance has rapidly risen and is roughly on par with our method. Both of them outperform EGNN by a considerable margin, which is consistent with that reported in their original paper. This further proves that the reason why SGNN fails to perform well under pixel supervision is caused by the uncertainty of 2D to 3D. EGNN is better than SGNN under 2D supervision because it predefines the direction of message passing which reduces the learning space as well. More importantly, our promising performance illustrates the effectiveness of incorporating strong mechanical priors for both 2D and 3D labels used. 
Our approach seems to excel in simulating solids, particularly elastic and rigid bodies. However, the SGNN method outperforms in simulating particulate matter like sand and viscous liquids. This discrepancy may stem from the presence of bond forces in our mechanical framework, constraining particles belonging to the same material.
\begin{table}[t]
    \centering
\scalebox{0.95}{
    \setlength\tabcolsep{0.5mm}{
\begin{tabular}{lcccccc}
\hline
\multicolumn{7}{c}{Given 3D GT Rollout MES $\times$ 10\textasciicircum{}2}                \\
Method & Plasticine & SandFall & Multi-Objs & FluidR & Bear  & \multicolumn{1}{l}{Fluids} \\ \hline
Ours   & \textbf{0.275}      & \textbf{0.0414}   & \textbf{0.239}      & 0.136  & 0.301 & \textbf{0.051}                      \\
SGNN*  & 0.268      & 0.0468   & 0.252      & \textbf{0.121}  & \textbf{0.282} & 0.062                      \\
EGNN*  & 0.614      & 0.127    & 0.568      & 0.318  & 0.705 & 0.143                    \\ \hline
\end{tabular}}}
\vspace{-0.175cm}
    \caption{Quantitative comparisons between our method and benchmarks on five scenarios in particle views.}
    \label{tab: 3D gt is given}
\vspace{-0.265cm}
\end{table}
\subsection{Detailed Qualitative Results in both render and particle views}
In this section, we report several additional qualitative results in Fig~\ref{fig: vissup 1} and Fig.~\ref{fig: vissup 2}. These figures include both particle view and render view of our method, EGNN$^*$, and DeVRF. The SGNN$^*$ is excluded since it performs worse than EGNN$^*$. More detailed results can be seen in our supplementary video. For the EGNN$^*$ and our method, we demonstrate both render and particle views to faithfully compare the predicted dynamics. For the DeVRF, we only report the rendering results because the particle view is not available for it. In addition, our method and EGNN$^*$ are trained on the training set and the reported results are evaluated on the test set. The DeVRF directly trained on the test sequences because it only can overfit a specific dynamic scene but cannot generalize to unobserved scenes. 

It can be observed from these figures that our method can generalize well to different initial shapes and conditions, especially when predicting long-term dynamics. While the EGNN$^*$ cannot precisely predict the mechanical behaviors between materials. Even though in some cases, such as BEAR and FluidR, the EGNN$^*$ can deliver plausible results at the early stage of interactions, the performance degrades drastically with the progressing deformation. The reconstructed scenes by DeVRF are optimized on the groundtruth data, but it only produces blur and vague images because of the spatially and temporally sparse-looking views. Dynamic NeRF methods only try to memorize certain sequences by rote and are difficult to understand realistic physics motions.  

We show a comparison of baselines for the Fluids dataset in Fig.~\ref{fig: liquidsup}. Our method preserves the basic trend of water flow, which other methods do not.

\subsection{Additional Demonstrations of Swapping Materials}
Our methodology introduces a novel capability for dynamic material pair substitution within pre-existing simulation environments. By predefining mechanical responses and employing a Graph Neural Network (GNN) solely for mapping deformations to interaction forces, we facilitate the modification of material interactions with minimal adjustments. This process involves substituting the parameters of the GNN kernel with those derived from alternative scenarios and altering the input $A_{ij}$, representing the adjacency matrix or interaction terms.

Figure~\ref{fig: change 1} illustrates this concept by substituting the original fluid-elastic interaction pair with a plastic-elastic pair in the Bear scenario, and a sand-elastic pair in the SandFall scenario, demonstrating the adaptability of our approach to simulate varied mechanical behaviors. Similarly, Figure~\ref{fig: change 2} presents another application of our method, where the sand soil material is replaced with elastic and plastic materials, leveraging GNN kernels trained in distinct contexts. These examples underscore our method's versatility in simulating diverse material behaviors through strategic parameter adjustments.
% \end{multicols}
% \twocolumn
% \begin{multicols}{2}
\section{Limitation}
The proposed method also has several limitations that need to be investigated in future research. The dynamic module is trained by the gradient propagating backward from image alignment, thus occlusion might be a significant issue. Future work can focus on learning particle-based dynamics from monocular videos with occluded objects. In addition, the proposed method only evaluates on simulation environment with simple shapes and appearances. In the future, we are going to explore real world scenes with complex geometries and textures. 
% \end{multicols}

% \section{Rationale}
% \label{sec:rationale}
% % 
% Having the supplementary compiled together with the main paper means that:
% % 
% \begin{itemize}
% \item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
% \item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
% \item When submitted to arXiv, the supplementary will already included at the end of the paper.
% \end{itemize}
% % 
% To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.https://www.overleaf.com/project/659cde01fe68e2088ae64463
